Observational Scaling Laws and the Predictability of Language Model Performance

Understanding how language model performance varies with scale is critical to benchmark and algorithm development. Scaling laws are one approach to building this understanding, but the requirement of training models across many different scales has limited their use. We propose an alternative, observational approach that bypasses model training and instead builds scaling laws from ~100 publically available models. Building a single scaling law from multiple model families is challenging due to large variations in their training compute efficiencies and capabilities. However, we show that these variations are consistent with a simple, generalized scaling law where language model performance is a function of a low-dimensional capability space, and model families only vary in their efficiency in converting training compute to capabilities. Using this approach, we show the surprising predictability of complex scaling phenomena: we show that several emergent phenomena follow a smooth, sigmoidal behavior and are predictable from small models; we show that the agent performance of models such as GPT-4 can be precisely predicted from simpler non-agentic benchmarks; and we show how to predict the impact of post-training interventions like Chain-of-Thought and Self-Consistency as language model capabilities continue to improve.

==> Tables/emerg_cap_quant_compare.tex <==
\yrnote{putt the table here because the error curve is not that neat due to non-smoothness, should we still use the plot?}
\begin{table}[h!]
    \centering
    \caption{Utilizing PC measures yields more accurate forecasts of LMs' emergent capabilities with 3 PCs generally being the best. The areas under the test error curves (AUE) as the training/test data size varies are measured to quantify the average forecasting errors (see error curves in \cref{fig:base_llm_emerg_cap_main_tasks_quant_analysis}). }
    \label{tab:emerg_cap_quant_compare}

    \small 
    
    \begin{tabular}{ll|c|c|c|c}
    \toprule
    \multicolumn{2}{c}{\textbf{Scale Measure}} & \textbf{Word Un.} & \textbf{Persian QA}  & \textbf{3-digit Sub.} & \textbf{2-digit Mul.} \\
    \midrule[\heavyrulewidth]
    \multirow{2}{*}{\raisebox{-0.5ex}[0pt][0pt]{Compute}} & Model Size & 2.92E-2 &  6.76E-3 & 2.28E-1 & 1.44E-1\\
    \cmidrule{2-6}
    & Training FLOPs & 1.11E-2 & 3.36E-3 & 1.03E-1 & 5.40E-2 \\
    \midrule[\heavyrulewidth]
    \multirow{4}{*}{\raisebox{-1.5ex}[0pt][0pt]{\makecell[l]{Principle\\Capabilities}}} & $\numpc = 1$ & 8.61E-3 & 3.43E-3 & 8.61E-2 & 4.41E-2 \\
    \cmidrule{2-6}
    & $\numpc = 2$ & 
    \textbf{4.91E-3} & 3.19E-3 & 4.57E-2 & 4.05E-2 \\
    \cmidrule{2-6}
    & $\numpc = 3$ & 5.46E-3  & \textbf{3.10E-3} & \textbf{3.61E-2} & \textbf{2.54E-2} \\
    \cmidrule{2-6}
    & $\numpc = 4$ & 5.88E-3   & 7.79E-3 & 4.32E-2 & 2.95E-2 \\
    \bottomrule
    \end{tabular}
\end{table}


==> Tables/property_comparison.tex <==
\begin{table}[t!]
    \centering
    \caption{Comparison between conventional and observational (ours) scaling laws.}
    \label{tab:property_comparison}

    \small
    
    \begin{tabularx}{0.95\textwidth}{l|>{\hsize=1\hsize}X|>{\hsize=1\hsize}X}
    \toprule
      & \multicolumn{1}{c|}{\textbf{Conventional}} & \multicolumn{1}{c}{\textbf{Observational}} \\
    \midrule
     \textbf{Cost} & training a large set of models across scales & evaluating available models \\
     \midrule 
     \textbf{Coverage} & a limited set of homogenous models with specific training recipe & publicly accessible models from heterogeneous sources for multi-dim. analysis \\
     \midrule 
     \textbf{Use case} & typically limited to scaling analysis of LM's pretraining loss & scaling analysis of various complex properties of LMs, \eg, agentic capabilities \\
     
    \bottomrule
    \end{tabularx}
\end{table}
\yrnote{not sure if this should be kept}
